Logic-Q: Improving Deep Reinforcement Learning-based Quantitative Trading via Program Sketch-based Tuning

Deep reinforcement learning (DRL) has revolutionized quantitative trading (Q-trading) by achieving decent performance without significant human expert knowledge. Despite its achievements, we observe that the current state-of-the-art DRL models are still ineffective in identifying the market trends, causing them to miss good trading opportunities or suffer from large drawdowns when encountering market crashes. To address this limitation, a natural approach is to incorporate human expert knowledge in identifying market trends. Whereas, such knowledge is abstract and hard to be quantified. In order to effectively leverage abstract human expert knowledge, in this paper, we propose a universal logic-guided deep reinforcement learning framework for Q-trading, called Logic-Q. In particular, Logic-Q adopts the program synthesis by sketching paradigm and introduces a logic-guided model design that leverages a lightweight, plug-and-play market trend-aware program sketch to determine the market trend and correspondingly adjusts the DRL policy in a post-hoc manner. Extensive evaluations of two popular quantitative trading tasks demonstrate that Logic-Q can significantly improve the performance of previous state-of-the-art DRL trading strategies.

==> tex/checklist.tex <==
\clearpage
\newpage
\section{Reproducibility Checklist}

This paper:
\begin{itemize}
[topsep=2pt,itemsep=2pt,partopsep=0ex,parsep=0ex,leftmargin=*]
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced \textbf{yes}
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \textbf{yes}
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper \textbf{yes}
\item Does this paper make theoretical contributions? \textbf{yes}

If yes, please complete the list below.

\item All assumptions and restrictions are stated clearly and formally. \textbf{yes}
\item All novel claims are stated formally (e.g., in theorem statements). \textbf{yes}
\item Proofs of all novel claims are included. \textbf{yes}
\item Proof sketches or intuitions are given for complex and/or novel results. \textbf{yes}
\item Appropriate citations to theoretical tools used are given. \textbf{yes}
\item All theoretical claims are demonstrated empirically to hold. \textbf{yes}
\item All experimental code used to eliminate or disprove claims is included. \textbf{yes}
\item Does this paper rely on one or more datasets? \textbf{yes}

If yes, please complete the list below.

\item A motivation is given for why the experiments are conducted on the selected datasets \textbf{yes}
\item All novel datasets introduced in this paper are included in a data appendix. \textbf{yes}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{yes}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textbf{yes}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textbf{yes}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \textbf{NA}
\item Does this paper include computational experiments? \textbf{yes}

If yes, please complete the list below.

\item Any code required for pre-processing data is included in the appendix. \textbf{yes}
\item All source code required for conducting and analyzing the experiments is included in a code appendix. \textbf{yes}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{yes}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \textbf{yes}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \textbf{yes}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textbf{yes}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \textbf{yes}
\item This paper states the number of algorithm runs used to compute each reported result. \textbf{yes}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textbf{yes}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textbf{no}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \textbf{yes}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \textbf{yes}
\end{itemize}

==> tex/discussion.tex <==
\section{DISCUSSION}
When scaling Logic-Q to real-world trading, it may encounter the challenges of the incompleteness of program sketch. The market dynamics is extremely complicated which may vary with many factors (\eg~asset types, global economic conditions, \etc). The program sketch we proposed and used in this work is not meant to be complete for market prediction, rather it is a proof-of-concept for the validity of the Logic-Q neural-symbolic framework. Therefore it might be invalid for some extreme market conditions that are not included in the logic of symbolic trend analyzer. This can be resolved by incorporating more human expertise regarding the market microstructure~\cite{bekaert2003emerging, spulber1996market,brock1992simple}.

==> tex/threats.tex <==
\section{THREATS TO VALIDITY}
The simulated trading environment setup adopted by previous baseline methods could be a threat to the validity of our results. We addressed this by trying our best to implement the real-world trading procedure. Specifically, we used the most realistic market data, diversified assets, and various financial instruments. We restricted the total capital that can be traded daily to effectively avoid market fluctuations. In order execution, we used TWAP for placing orders, which effectively ensures order fulfillment and minimizes market impact. 
% Additionally, we applied fair transaction fees and slippage. During the testing period, each market experienced bull, bear, and sideways trends, demonstrating that our strategy can achieve stable returns across different market cycles. The variations of the trained DRL policies could be another threat to the validity of our results. We resolve this by reporting the mean and standard deviation of the results average over 5 random seeds.
